Group Generalized Mean Pooling for Vision Transformer

Vision Transformer (ViT) extracts the final representation from either class token or an average of all patch tokens, following the architecture of Transformer in Natural Language Processing (NLP) or Convolutional Neural Networks (CNNs) in computer vision. However, studies for the best way of aggregating the patch tokens are still limited to average pooling, while widely-used pooling strategies, such as max and GeM pooling, can be considered. Despite their effectiveness, the existing pooling strategies do not consider the architecture of ViT and the channel-wise difference in the activation maps, aggregating the crucial and trivial channels with the same importance. In this paper, we present Group Generalized Mean (GGeM) pooling as a simple yet powerful pooling strategy for ViT. GGeM divides the channels into groups and computes GeM pooling with a shared pooling parameter per group. As ViT groups the channels via a multi-head attention mechanism, grouping the channels by GGeM leads to lower head-wise dependence while amplifying important channels on the activation maps. Exploiting GGeM shows 0.1%p to 0.7%p performance boosts compared to the baselines and achieves state-of-the-art performance for ViT-Base and ViT-Large models in ImageNet-1K classification task. Moreover, GGeM outperforms the existing pooling strategies on image retrieval and multi-modal representation learning tasks, demonstrating the superiority of GGeM for a variety of tasks. GGeM is a simple algorithm in that only a few lines of code are necessary for implementation.

==> table/tab_classification_small.tex <==
\begin{table}[]
\begin{adjustbox}{width=0.9\columnwidth,center}
\centering
\begin{tabular}{lcc>{\columncolor{Light}}c>{\columncolor{Light}}cc}
\toprule
         & Class & Average & \multicolumn{2}{>{\columncolor{Light}}c}{\textit{GGeM}} & Reported \\ \cline{2-6} 
Method   & Acc.  & Acc.    & Acc.       & (Gain)        & Acc.  \\
\midrule
\textit{\textbf{ViT-S/16}} &       &         &            &             &       \\
Scratch  & 80.0  & 80.4    & \textbf{80.7}       & \textcolor{Green}{(+0.3)}      & 79.9$^\ddagger$  \\
\midrule
\textit{\textbf{ViT-B/16}} &       &         &            &             &       \\
Scratch  & 82.4  & 82.4    & \textbf{82.7}       & \textcolor{Green}{(+0.3)}      & 81.8$^\ddagger$  \\
MAE      & -     & 83.5    & \textbf{83.9}       & \textcolor{Green}{(+0.4)}      & 83.6  \\
BeiT$^\dagger$     & -     & 83.6    & \textbf{83.8}       & \textcolor{Green}{(+0.2)}      & 83.7  \\
SimMIM   & -     & 83.7    & \textbf{84.0}       & \textcolor{Green}{(+0.3)}      & 83.8  \\
Data2Vec & -     & 84.0    & \textbf{84.3}       & \textcolor{Green}{(+0.3)}      & 84.2  \\
\midrule
\textit{\textbf{ViT-L/16}} &       &         &            &             &       \\
MAE      & -     & 85.8    & \textbf{86.0}       & \textcolor{Green}{(+0.2)}      & 85.9  \\
BeiT$^\dagger$     & -     & 85.9    & \textbf{86.2}       & \textcolor{Green}{(+0.3)}      & 86.0  \\
Data2Vec & -     & 86.5    & \textbf{86.7}       & \textcolor{Green}{(+0.2)}      & 86.6  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Scratch training (Scratch) and fine-tuning with SSL models for ImageNet-1K classification.} Every SSL model are pre-trained with ImageNet-1K, except BeiT~\cite{bao2021beit} with $^\dagger$ used ImageNet-22K. We report top-1 accuracy (Acc.), with ``Gain'', which is a comparison between Average and GGeM Pooling. ``Reported'' indicates reported score in the original paper. $^\ddagger$ denotes scores from DeiT~\cite{touvron2021deit}.\vspace{-3mm}}
\label{table:classification}
\end{table}



==> table/tab_imagenet_config.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=1.0\textwidth,center}
\centering
\begin{tabular}{lcccccc}
\toprule
Config                    & Scratch                      & MAE                           & BeiT                          & SimMIM                        & Data2Vec                      & Linear probing    \\
\midrule
Initial p                 & 5                            & 5 (B), 2 (L)                   & 5                             & 4                             & 3                             & 3                 \\
Optimizer                 & AdamW                        & AdamW                         & AdamW                         & AdamW                         & AdamW                         & LARS              \\
Learning rate             & 8e-3                         & 2e-3                          & 4e-3                          & 5e-3                          & 4e-3 (B), 5e-3 (L)            & 0.64              \\
Weight decay              & 0.3                          & 0.05                          & 0.05                          & 0.05                          & 0 (B), 0.05 (L)               & 0                 \\
Optimizer momentum        & $\beta_1$, $\beta_2$ = 0.9, 0.95 & $\beta_1$, $\beta_2$ = 0.9, 0.999 & $\beta_1$, $\beta_2$ = 0.9, 0.999 & $\beta_1$, $\beta_2$ = 0.9, 0.999 & $\beta_1$, $\beta_2$ = 0.9, 0.999 & 0.9               \\
Layer decay       & 0.75                         & 0.65 (B), 0.75 (L)             & 0.65 (B), 0.75 (L)             & 0.65                          & 0.65                          & -                 \\
Batch size                & 4096                         & 1024                          & 1024                          & 2048                          & 1024                          & 16384             \\
LR schedule    & cosine decay                 & cosine decay                  & cosine decay                  & cosine decay                  & cosine decay                  & cosine decay      \\
Warmup epochs             & 20                           & 5 (B), 10 (L)                & 20 (B), 5 (L)                 & 20                            & 10 (B), 5 (L)                 & 10                \\
Traning epochs            & 300                          & 100 (B), 50 (L)                & 100 (B), 50 (L)               & 100                           & 100 (B), 50 (L)                & 90                \\
Augmentation              & RandAug (9, 0.5)             & RandAug (9, 0.5)              & RandAug (9, 0.5)              & RandAug (9, 0.5)              & RandAug (9, 0.5)              & RandomResizedCrop \\
Label smoothing           & 0.1                          & 0.1                           & 0.1                           & 0.1                           & 0.1                           & -                 \\
Mixup                     & 0.8                          & 0.8                           & 0.8                           & 0.8                           & 0.8                           & -                 \\
Cutmix                    & 1.0                          & 1.0                           & 1.0                           & 1.0                           & 1                             & -                 \\
Drop path                 & 0.1                          & 0.1 (B), 0.2 (L)              & 0.1 (B), 0.2 (L)              & 0.1                           & 0.2 (B), 0.25 (L)             & -                 \\
Exp. moving average & 0.9999                       & -                             & -                             & -                             & -                             & -                 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Hyper-parameter setting for ImageNet-1K classification.}}
\label{table:supp_class_param}
\end{table*}

==> table/tab_ret_clip_config.tex <==
\begin{table*}[t]
    \begin{subtable}[h]{0.5\textwidth}
        \begin{adjustbox}{width=0.8\textwidth,center}
        \centering
        \begin{tabular}{lc}
        \toprule
        Config                 & Value                             \\
        \midrule
        Initial p              & 3                                 \\
        Model                  & ViT-B/16                          \\
        Optimizer              & AdamW                             \\
        Learning rate          & 2e-3                              \\
        Weight decay           & 0.05                              \\
        Optimizer momentum     & $\beta_1$, $\beta_2$ = 0.9, 0.999 \\
        Layer-wise LR decay    & 0.65                              \\
        Batch size             & 128                               \\
        Learning rate schedule & cosine decay                      \\
        Warmup epochs          & 5                                 \\
        Traning epochs         & 100 (Cars, CUB), 50 (SOP)         \\
        Augmentation           & RandAug (9, 0.5)                  \\
        Drop path              & 0.1                               \\
        Base learning rate     & 4e-3                              \\
        Proxy LR scale         & 100                              \\
        \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Image retrieval setting}
    \label{table:ret_param}
    \end{subtable}
\hfill
    \begin{subtable}[h]{0.5\textwidth}
        \begin{adjustbox}{width=0.7\textwidth,center}
        \centering
        \begin{tabular}{lc}
        \toprule
        Config                 & Value                            \\
        \midrule
        Initial p              & 3                                \\
        Model                  & ViT-B/32                         \\
        Optimizer              & AdamW                            \\
        Learning rate          & 1e-3                             \\
        Weight decay           & 0.2                              \\
        Optimizer momentum     & $\beta_1$, $\beta_2$ = 0.9, 0.98 \\
        Batch size             & 4080                             \\
        Learning rate schedule & cosine decay                     \\
        Warmup steps           & 3500                             \\
        Traning epochs         & 25                               \\
        Augmentation           & RandomResizedCrop               \\
        \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Multi-modal representation learning setting}
    \label{table:mm_param}
    \end{subtable}
\caption{\textbf{Hyper-parameter settings for image retrieval and multi-modal representation learning.}}
\label{table:params}
\end{table*}

==> tex/99_algorithm.tex <==
\begin{algorithm}[t]
\caption{GGeM: PyTorch-like Pseudo-code}
\label{alg:code}
\algcomment{
\textbf{Notes}: \texttt{clamp} is a function to clamp all elements into the range [min, max].
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
\begin{lstlisting}[language=python]
# x: output tensor of the last Transformer block (batch size x tokens x dimension)
# p_params: pooling parameters, the number of pooling parameters is the same with groups
# groups: number of groups
# eps: minimum value for clamping
def GGeM(x):
    x = x[:, 1:, :] # Remove class token
    
    b, t, d = x.shape
    e = d // groups
    x = x.reshape((b, t, e, groups))

    x = x.clamp(min=eps).pow(p_params)
    x = x.mean(dim=1)
    x = x.pow(1./p_params)

    x = x.reshape((b, d))
    return x

\end{lstlisting}
\end{algorithm}
